Beyond the Binary: Capturing Diverse Preferences With Reward Regularization

Large language models (LLMs) are increasingly deployed via public-facing interfaces to interact with millions of users, each with diverse preferences. Despite this, preference tuning of LLMs predominantly relies on reward models trained using binary judgments where annotators select the preferred choice out of pairs of model outputs. In this work, we argue that this reliance on binary choices does not capture the broader, aggregate preferences of the target user in real-world tasks. We propose a taxonomy that identifies two dimensions of subjectivity where different users disagree on the preferred output-namely, the Plurality of Responses to Prompts, where prompts allow for multiple correct answers, and the Indistinguishability of Responses, where candidate outputs are paraphrases of each other. We show that reward models correlate weakly with user preferences in these cases. As a first step to address this issue, we introduce a simple yet effective method that augments existing binary preference datasets with synthetic preference judgments to estimate potential user disagreement. Incorporating these via a margin term as a form of regularization during model training yields predictions that better align with the aggregate user preferences.

==> related.tex <==
\section{Related Work}
\label{sec:related}

\begin{itemize}
    \item \citet{rame2024rewarded} handle diverse rewards by training multiple reward models and averaging their parameter values, akin to model soups \cite{wortsman2022model}
    \item \citet{chakraborty2024maxmin} maximize the minimum utility for all subpopulations within a mixture of diverse preferences
    \item \cite{jang2023personalized}
    \item \cite{bakker2022fine}
\end{itemize}
